Consistent Query Answering over SHACL Constraints

The Shapes Constraint Language (SHACL) was standardized by the World Wide Web as a constraint language to describe and validate RDF data graphs. SHACL uses the notion of shapes graph to describe a set of shape constraints paired with targets, that specify which nodes of the RDF graph should satisfy which shapes. An important question in practice is how to handle data graphs that do not validate the shapes graph. A solution is to tolerate the non-validation and find ways to obtain meaningful and correct answers to queries despite the non-validation. This is known as consistent query answering (CQA) and there is extensive literature on CQA in both the database and the KR setting. We study CQA in the context of SHACL for a fundamental fragment of the Semantic Web query language SPARQL. The goal of our work is a detailed complexity analysis of CQA for various semantics and possible restrictions on the acceptable repairs. It turns out that all considered variants of the problem are intractable, with complexities ranging between the first and third level of the polynomial hierarchy.

==> cqa-shacl.tex <==
\section*{Old}
\section{Problems studied here}
\label{sect:cqa}

The basic problem for given query language $\mathcal{L}$ and pre-order 
$\preceq$ on repairs is the 
following \cqa problem ($\mathcal{Q}\in \{\exists, \forall, \cap\}$): 

\problemdef{\LPrecQ}{A graph $G$, a shape document $(C,T)$, and a set of hypotheses $H$
      as well as a query $Q \in \mathcal{L}$ and a mapping $\mu$}{Is $\mu$ a solution of $Q$ over a / every / the intersection of all $\preceq$-minimal repaired graphs $G_R$ of $G$ w.r.t.\ $(C,T,H)$}

% \begin{problem}
%       \problemtitle{\cqa$(\mathcal{L},\preceq, (\forall/ \exists /\cap))$}
%       \probleminstance{A graph $G$, a shape document $(C,T)$, and a set of hypotheses $H$
%       as well as a query $q \in \mathcal{L}$ and a mapping $\mu$.}
%       \problemquestion{Is $\mu$ a solution of $q$ in every / a / the intersection of all $\preceq$-minimal repair $(A,D)$ of $G$ w.r.t.\ $(C,T,H)$?}
% \end{problem}

\todo[inline]{CM: The intersection of repairs need not be a repair itself. Is that a problem? Should we address this?}


We get several variants of the \cqa-$\mathcal{L}$ problem by considering
various query languages $\mathcal{L}$ and pre-orders $\preceq$.

\begin{itemize}
    \item various query languages:  basic graph patterns (BGPs), 
    BGPs with projection ($\pi$-BGPs), well-designed pattern trees
    (WDPTs), and WDPTs with projectin ($\pi$-WDPTs);
    \item various minimality conditions on the repairs: 
    any repairs ($=$), subset-minimal repairs ($\subseteq$), cardinality-minimal  ($\leq$) repairs;
    \item possibly also various semantics (i.e., notions of models): in the first place, we only study supported models; later, we will also consider
    stable models and well-founded model.
\end{itemize}


In total, we thus get 36 problems for each semantics (to begin with, we
consider only 1 semantics, namely supported models):

\todo[inline,caption={}]{CM: Further worthwhile options: 
\begin{itemize}
    \item $H$ fixed to $\emptyset$ 
    \item Union over all repair (extremely brave reasoning) \shqip{If a $\mu$ is a solution over the union of all repairs, then what insights would this give wrt to a repair? Note that if $\mu$ is a solution over the intersection of repairs, then it is a solution in every repair, and in some repair (for positive queries). This holds under the assumption that repair here means the resulting repaired data graph.}
\end{itemize}
}

\smallskip

\bgpEqu, \bgpSubs, \bgpCard

\bgpProjEqu, \bgpProjSubs, \bgpProjCard

\wdptEqu, \wdptSubs, \wdptCard


\wdptProjEqu, \wdptProjSubs, \wdptProjCard

\smallskip

\bgpEquEx, \bgpSubsEx, \bgpCardEx

\bgpProjEquEx, \bgpProjSubsEx, \bgpProjCardEx

\wdptEquEx, \wdptSubsEx, \wdptCardEx


\wdptProjEquEx, \wdptProjSubsEx, \wdptProjCardEx

\smallskip

\bgpEquIn, \bgpSubsIn, \bgpCardIn

\bgpProjEquIn, \bgpProjSubsIn, \bgpProjCardIn

\wdptEquIn, \wdptSubsIn, \wdptCardIn


\wdptProjEquIn, \wdptProjSubsIn, \wdptProjCardIn

\medskip

\begin{table}[h]
\centering
\caption{Cautious Reasoning ($\forall$)}
\begin{tabular}{|c|c|c|c|}
\hline
& $=$ & $\subseteq$ & $\leq$ \\
\hline
\textsc{Bgp}        & \green{\conp} / \conp             & \green{\pitwo} / \pitwo           & \green{\thetatwo} / \thetatwo \\
$\pi$-\textsc{Bgp}  & \conp / \purple{\pitwo}           & \pitwo / \red{\pitwo}                   & \thetatwo / \purple{\pitwo} \\
\textsc{Wdpt}       & \conp / \red{\conp}               & \pitwo / \red{\pitwo}             & \thetatwo / \red{\thetatwo} \\
$\pi$-\textsc{Wdpt} & \red{\conp} / \purple{\pithree}   & \red{\pitwo} / \purple{\pithree}  & \red{\thetatwo} / \purple{\pithree} \\
\hline
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Very Cautious Reasoning ($\cap$)}
\begin{tabular}{|c|c|c|c|}
\hline
& $=$ & $\subseteq$ & $\leq$ \\
\hline
\textsc{Bgp}        & \green{\conp} / \red{\conp}               & \green{\pitwo} / \pitwo                   & \green{\thetatwo} / \thetatwo \\
$\pi$-\textsc{Bgp}  & \red{\conp} / \purple{\thetatwo}          & \pitwo / \red{\pitwo}                     & \thetatwo  / \red{\thetatwo}  \\
\textsc{Wdpt}       & \purple{\DP} / \purple{\thetatwo}         & \green{\DPtwo} / \red{\DPtwo}             & \thetatwo / \red{\thetatwo} \\
$\pi$-\textsc{Wdpt} & \purple{\thetatwo} / \purple{\sigmatwo}   & \green{\thetathree} / \red{\thetathree}   & \red{\thetatwo} / \purple{\sigmatwo} \\
\hline
\end{tabular}
\end{table}



\begin{table}[h]
\centering
\caption{Brave Reasoning ($\exists$)}
\begin{tabular}{|c|c|c|c|}
\hline
& $=$ & $\subseteq$ & $\leq$ \\
\hline
\textsc{Bgp}        & \green{\np} / \np             & \green{\sigmatwo} / \sigmatwo & \green{\thetatwo} / \thetatwo \\
$\pi$-\textsc{Bgp}  & \np / \red{\np}               & \sigmatwo / \sigmatwo         & \thetatwo / \red{\thetatwo} \\
\textsc{Wdpt}       & \np / \green{\sigmatwo}       & \sigmatwo / \sigmatwo         & \thetatwo / \green{\sigmatwo} \\
$\pi$-\textsc{Wdpt} & \red{\np} / \red{\sigmatwo}   & \sigmatwo / \red{\sigmatwo}   & \red{\thetatwo} / \red{\sigmatwo} \\
\hline
\end{tabular}
\end{table}

\todo[inline]{CM: for myself: Check arguments again (multiple co questions).}

\todo[inline]{RP: These problem names are all defined by macros. So it should be no problem if we want to change the names.}

\noindent
Moreover, for each problem, we may consider data complexity or combined complexity.
That is, for data complexity, we consider all parts of the instance apart from the graph $G$ 
as fixed. In principle we could of course also consider 3 components 
(data, constraints, query) of the input separately and 
consider 0, 1, or 2 of these components as fixed (in the style of \cite{DBLP:conf/icdt/ArmingPS16}).


\section{Upper Bounds}
\label{sect:UpperBounds}

\subsection{Query language: BGPs}

First, note that without projection, there is no difference between cautious and very cautious reasoning.
If the relevant tuples are in all repairs, they clearly also lie in the intersection of all repairs.

\begin{theorem}
\label{thm:bgpEqu}
The problems \bgpEqu and \bgpEquIn are in \conp data complexity and 
combined complexity.   
\end{theorem}


\todo[inline]{RP: I am not 100\% sure that the definition of CQA is okay in the case that 
there exists no repair of $G$ at all. Is it okay that, in this case, every mapping $\mu$ 
would be a solution? Or should we add the \np-check that there exists at least one repair? 
In this case, the problem  \bgpEqu would be in \DP (and hopefully \DP-complete).}




\begin{theorem}
\label{thm:bgpSubs}
The problems \bgpSubs and \bgpSubsIn are in \pitwo data complexity and 
combined complexity.   
\end{theorem}






\begin{theorem}
\label{thm:bgpCard}
The problems \bgpCard and \bgpCardIn are in \thetatwo data complexity and 
combined complexity.   
\end{theorem}


\begin{theorem}
\label{thm:bgpInhardness}
The following statements are true for data complexity and 
combined complexity:
\begin{itemize}
    \item \bgpEqu and \bgpEquIn are \conp-hard.
    \item \bgpSubs and \bgpSubsIn are \pitwo-hard.
    \item \bgpCard and \bgpCardIn are \thetatwo-hard.
\end{itemize}  
\end{theorem}



\begin{theorem}
\label{thm:bgpExhardness}
The following statements are true for data complexity and 
combined complexity:
\begin{itemize}
    \item \bgpEquEx is \np-complete.
    \item \bgpSubsEx is \sigmatwo-complete.
    \item \bgpCardEx is \thetatwo-complete.
\end{itemize}  
\end{theorem}


% \begin{proof}

% The simple (single atom) query asking whether a $B(a)\in A$ is an answer over all repairs is the same as asking whether $B(a)$ is a necessary addition. 
% This is already $\mathsf{coNP}$-hard (Theorem 4. of the KR paper; we could also use (the co of) relevant add which is $\mathsf{NP}$-complete \cite{DBLP:conf/kr/AhmetajDOPSS21}).
% \end{proof}

% \todo[inline]{Proof is written badly. But the idea is that $\mathsf{co}(=/\leq/\subseteq$)\textsc{RelavantDelete} can easily be reduced to to CQA(\textsc{Bgp}$(=/\leq/\subseteq)$)}

% \begin{theorem}
% \label{thm:bgpSubs}
% The problem  data complexity and 
% combined complexity.   
% \end{theorem}

% \begin{proof}
% The simple (single atom) query asking whether a $B(a)\in G$ is an answer over all repairs is the same as asking whether $B(a)$ cannot be removed.
% The co-problem of this is to ask whether $B(a)$ is a relevant deletion, i.e., if there is a minimal repair such that $B(a)\in D$
% This is already \sigmatwo-hard (Theorem 5. of the KR paper \cite{DBLP:conf/kr/AhmetajDOPSS21}).
% \end{proof}

% \begin{theorem}
% \label{thm:bgpCard}
% The problem  data complexity and 
% combined complexity.   
% \end{theorem}

% \begin{proof}

% The simple (single atom) query asking whether a $B(a)\in G$ is an answer over all repairs is the same as asking whether $B(a)$ cannot be removed.
% The co-problem of this is to ask whether $B(a)$ is a relevant deletion, i.e., if there is a minimal repair such that $B(a)\in D$
% This is already \thetatwo-hard (Theorem 5. of the KR paper \cite{DBLP:conf/kr/AhmetajDOPSS21}).
% \end{proof}


\subsection{Query language: BGPs with projection}

As we have seen above, the check if a mapping $\mu$ is a solution of a BGP $q$ over a graph 
(or a  repair thereof) is very easy: we just have to check if all triples in $q \mu$ 
are contained in the graph or repair. If we now consider BGPs with projection, then the check if 
$\mu$ is a solution is more involved: 
for cautious and brave reasoning, given a repair, we now have to check if $\mu$ can be extended to a mapping $\nu$
covering also the existentially quantified variables, so that all triples in $q \nu$ are contained in the graph or repair. 
In terms of data complexity, this is still feasible in polynomial time. 
For very cautious reasoning, we have to determine the extension before selecting the repair.
However, in terms of data complexity, we can compute all polynomially many extensions and then guess one repair per extension at the same time. 
Thus, here, the complexity also does not increase.
When only asking for the existence of a repair over which the query evaluates to true for $\mu$, the complexity even remains the same for combined complexity as we can guess the values for the existentially quantified variables of the query at the same time we guess the repair.

\begin{theorem}
The following statements are true for data complexity:
\begin{itemize}
    \item \bgpProjEqu and \bgpProjEquIn are \conp-complete.
    \item \bgpProjSubs and \bgpProjSubsIn are \pitwo-complete.
    \item \bgpProjCard and \bgpProjCardIn are \thetatwo-complete.
\end{itemize} 

Moreover, the following statements are true for data and combined complexity:

\begin{itemize}
    \item \bgpProjEquEx is \np-complete.
    \item \bgpProjSubsEx is \sigmatwo-complete.
    \item \bgpProjCardEx is \thetatwo-complete.
\end{itemize} 
\end{theorem}

However, for combined complexity and cautious reasoning, the existential variables potentially add the need for another non-deterministic guess.
Therefore, below, we only consider combined complexity. It turns out that, in this case, 
all problems \bgpProjEqu, \bgpProjSubs, and \bgpProjCard end up in \pitwo  
combined complexity. We now consider queries $q$ of the form
$q = (\exists \hat y) \, p(\hat x, \hat y)$ and test if a mapping
$\mu$ with $dom(\mu)= \hat x$ is a consistent answer.


\begin{theorem}
\label{thm:bgpProj}
The problems 
\bgpProjEqu, \bgpProjSubs, \bgpProjCard are in \pitwo combined complexity.   
\end{theorem}


\begin{theorem}
\label{thm:bgpProj}
\bgpProjEqu, \bgpProjSubs, \bgpProjCard are \pitwo-hard combined complexity.
\end{theorem}

\todo[inline]{Note that the document can be fixed. We only need combined complexity to adapt the query ($v_1,v_n$ have to be fixed constant vertices of $G'.$).}


Furthermore, for combined complexity and very cautious reasoning, we can start by computing the intersection over all repairs.
This only requires polynomial calls to single atom \textsc{Bgp} queries.
Hence there is no increase in the complexity at this point.
Then, the query has to be answered over the intersection which takes \np time as $\pi$-\textsc{Bgp} is \np-complete.

\begin{theorem}
\label{thm:bgpProjInhardness}
The following statements are true for combined complexity:
\begin{itemize}
    \item \bgpProjEquIn is \thetatwo-complete.
    \item \bgpProjSubsIn is \pitwo-complete.
    \item \bgpProjCardIn is \thetatwo-complete.
\end{itemize}  
\end{theorem}

\subsection{Query language: WDPTs}

Also for WDPTs, the data complexity is the same as for BGPs. 
However, for
the combined complexity, we now have to take another reason why $\mu$ is {\em not}
a solution into account: it may happen that $\mu$ matches all triples of $q$
into $(G \setminus D) \cup A$ but $\mu$ 
can be extended to a mapping $\lambda$ that
also matches all triples in the OPT-part into $(G \setminus D) \cup A$.
Hence, checking that $\mu$ is not a solution of $q$ requires additional power. 
However, as we show below, this does not add to the complexity of BGPs for cautious reasoning. 
Intuitively, for cautious reasoning, this is due to the fact that we can guess the extension $\lambda$ together with the 
repair in which $\mu$ is not a solution. 
For very cautious reasoning, we have to be a bit more careful and the complexity only remains the same for \wdptSubsIn.
We now consider queries $q$ of the form 
$q = p(\hat x)$ OPT $r(\hat x', \hat z)$ with $\hat x' \subseteq \hat x$ 
and test if a mapping $\mu$ with $dom(\mu)= \hat x$ is a consistent answer.

\begin{theorem}
\label{thm:wdpt}
The following statements are true for data complexity:
\begin{itemize}
    \item \wdptEquEx is \np-complete.
    \item \wdptSubsEx is \sigmatwo-complete.
    \item \wdptCardEx is \thetatwo-complete.
    % \item \wdptEquIn is \conp-complete
    % \item \wdptSubsIn is \pitwo-complete
\end{itemize}  
However, the following statements are true for data and combined complexity:
\begin{itemize}
    \item \wdptEqu is \conp-complete.
    \item \wdptSubs is \pitwo-complete.
    \item \wdptCard and \wdptCardIn are \thetatwo-complete.
\end{itemize}   
\end{theorem}


On the other hand, for brave reasoning, this in fact does make a difference.

\begin{theorem}
\label{thm:wdpt}
\wdptEquEx, \wdptSubsEx, and \wdptCardEx are \sigmatwo-complete combined complexity.
\end{theorem}



\begin{theorem}
The following statements are true for data complexity:
\begin{itemize}
    \item \wdptEquIn is \DP-complete.
    \item \wdptSubsIn is \DPtwo-complete.
\end{itemize}
The following statements are true for combined complexity:
\begin{itemize}
    \item \wdptEquIn is \thetatwo-complete.
    \item \wdptSubsIn is \DPtwo-complete.
\end{itemize}
\end{theorem}

\subsection{Query language: WDPTs with projection}

Finally, we also study the complexity of 
consistent query answering 
of WDPTs with projection. Again, only the combined complexity is of interest, 
since the data complexity remains the same as for the much simpler queries 
BGPs (with or without projection) and WDPTs.
For brave reasoning, we can guess the values of the existential variables at the start and hence, as we are already in \sigmatwo, the complexity remains the same.
For very cautious reasoning, again, we can first compute the intersection of all repairs, again via single-atom BGP queries.
Then, we can solve the $\pi$-WDPT query.
For $=$- and $\leq$-minimal repairs the complexity of answering a $\pi$-WDPT overshadows the remainder.

\begin{theorem}
\label{thm:wdpt}
The following statements are true for data complexity:
\begin{itemize}
    \item \wdptProjEqu is \conp-complete.
    \item \wdptProjSubs is \pitwo-complete.
    \item \wdptProjEquEx is \np-complete.
    \item \wdptProjSubsEx is \sigmatwo-complete.
    \item \wdptProjCard and \wdptProjCardEx are \thetatwo-complete.
\end{itemize}   
Furthermore, \wdptProjEquEx, \wdptProjSubsEx, and \wdptProjCardEx are \sigmatwo-complete combined complexity.
\end{theorem}

However, for combined complexity, we climb even further in the polynomial hierarchy.

\begin{theorem}
\label{thm:wdptProj}
The problems \wdptProjEqu, \wdptProjSubs, and 
\wdptProjCard 
are in \pithree combined complexity.
\end{theorem}


\begin{theorem}
\label{thm:wdptProj}
The problems \wdptProjEqu, \wdptProjSubs, and \wdptProjCard are \pithree-hard combined complexity.
\end{theorem}

\begin{theorem}
The following statements are true for data complexity:
\begin{itemize}
    \item \wdptProjEquIn is \thetatwo-complete.
    \item \wdptProjSubsIn is \thetathree-complete.
    \item \wdptProjCardIn is \thetatwo-complete.
\end{itemize}
The following statements are true for combined complexity:
\begin{itemize}
    \item \wdptProjEquIn is \sigmatwo-complete.
    \item \wdptProjSubsIn is \thetathree-complete.
    \item \wdptProjCardIn is \sigmatwo-complete.
\end{itemize}
\end{theorem}





\section{Max-Variants of Consistent Query Answering}
\label{sect:max}

We now consider consistent query answering for settings where it is not 
guaranteed that a repair of $G$ w.r.t.\ $((C,T),H)$ for shape document $(C,T)$ and set of hypotheses $H$ exists. 
One approach (\red{citation?}) in this case is to relax the notion of repairs and to 
aim at satisfying the maximum number of targets. Formally, given a graph $G$, 
a shape document $(C,T)$ and a set of hypotheses $H$, 
we define a {\em max-repair} of $G$ w.r.t.\ $((C,T), H)$ as 
a pair $(A,D)$ satisfying

\begin{itemize}
\item $A \subseteq H$,  $D \subseteq G$,
\item there exists $T' \subseteq T$ such that $(A,D)$ is a repair 
of $G$ w.r.t.\ $((C,T'),H)$,
\item  for every $T'' \subseteq T$   with $|T''| > |T'>$, there exists no repair 
of $G$ w.r.t.\ $((C,T''), H)$.
\end{itemize}

We thus consider the following max-variant \mcqa of the consistent query answering 
problem for  given query language $\mathcal{L}$ and pre-order 
$\preceq$ on repairs:

\problemdef{\mcqa$(\mathcal{L},\preceq, (\forall/ \exists /\cap))$}{A graph $G$, a shape document $(C,T)$, and a set of hypotheses $H$
        as well as a query $q \in \mathcal{L}$ and a mapping $\mu$}{Is $\mu$ a solution of $q$ in every / a / the intersection of all $\preceq$-minimal max-repair(s) $(A,D)$ of $G$ w.r.t.\ $((C,T),H)$}
% \begin{problem}
%       \problemtitle{\mcqa$(\mathcal{L},\preceq, (\forall/ \exists /\cap))$}
%       \probleminstance{A graph $G$, a shape document $(C,T)$, and a set of hypotheses $H$
%         as well as a query $q \in \mathcal{L}$ and a mapping $\mu$.}
%       \problemquestion{Is $\mu$ a solution of $q$ in every / a / the intersection of all $\preceq$-minimal max-repair $(A,D)$ of $G$ w.r.t.\ $(C,T,H)$?}
% \end{problem}


Analogously to the basic problem \cqa-$\mathcal{L}$, we get 36 variants of the 
\mcqa-$\mathcal{L}$ problem by considering
4 query languages $\mathcal{L}$ 
(namely BGPs, $\pi$-BGPs, WDPTs, and $\pi$-WDPTs), 
3 pre-orders $\preceq$ (namely $=$, $\subseteq$, and $\leq$), 
and 3 semantics (namely cautions, intersection, and brave):


\smallskip

\mbgpEqu, \mbgpSubs, \mbgpCard

\mbgpProjEqu, \mbgpProjSubs, \mbgpProjCard

\mwdptEqu, \mwdptSubs, \mwdptCard

\mwdptProjEqu, \mwdptProjSubs, \mwdptProjCard

\smallskip

\mbgpEquEx, \mbgpSubsEx, \mbgpCardEx

\mbgpProjEquEx, \mbgpProjSubsEx, \mbgpProjCardEx

\mwdptEquEx, \mwdptSubsEx, \mwdptCardEx

\mwdptProjEquEx, \mwdptProjSubsEx, \mwdptProjCardEx

\smallskip

\mbgpEquIn, \mbgpSubsIn, \mbgpCardIn

\mbgpProjEquIn, \mbgpProjSubsIn, \mbgpProjCardIn

\mwdptEquIn, \mwdptSubsIn, \mwdptCardIn

\mwdptProjEquIn, \mwdptProjSubsIn, \mwdptProjCardIn

\medskip
\noindent
The complexities of these 36 problems (data/combined complexity) are summarized in
the 3 Tables \ref{tab:MaxCautious}, \ref{tab:MaxVeryCautious}, and \ref{tab:MaxBrave}, 

\begin{table}[h]
\centering
\caption{Cautious Reasoning ($\forall$)}
\label{tab:MaxCautious}
\begin{tabular}{|c|c|c|c|}
\hline
& $=$ & $\subseteq$ & $\leq$ \\
\hline
\textsc{Bgp} & \purple{\bh} / \purple{\thetatwo}  & \pitwo / \pitwo & \thetatwo / \thetatwo \\
$\pi$-\textsc{Bgp} & \purple{\bh} / \pitwo  & \pitwo / \pitwo & \thetatwo / \pitwo \\
\textsc{Wdpt} & \purple{\bh} / \purple{\thetatwo}  & \pitwo / \pitwo & \thetatwo / \thetatwo \\
$\pi$-\textsc{Wdpt} & \purple{\bh} / \pithree  & \pitwo / \pithree & \thetatwo / \pithree \\
\hline
\end{tabular}
\end{table}


\begin{table}[h]
\centering
\caption{Very Cautious Reasoning ($\cap$)}
\label{tab:MaxVeryCautious}
\begin{tabular}{|c|c|c|c|}
\hline
& $=$ & $\subseteq$ & $\leq$ \\
\hline
\textsc{Bgp} &  \purple{\bh} / \purple{\thetatwo}  & \pitwo / \pitwo & \thetatwo / \thetatwo \\
$\pi$-\textsc{Bgp} &  \purple{\bh} / \thetatwo & \pitwo / \pitwo & \thetatwo  / \thetatwo  \\
\textsc{Wdpt} &  \purple{\bh} / \thetatwo & \DPtwo / \DPtwo &  \thetatwo / \thetatwo \\
$\pi$-\textsc{Wdpt} & \thetatwo / \sigmatwo & \pitwo? / \pithree? &  \thetatwo / \sigmatwo \\
\hline
\end{tabular}
\end{table}

\begin{table}[h]
\centering
\caption{Brave Reasoning ($\exists$)}
\label{tab:MaxBrave}
\begin{tabular}{|c|c|c|c|}
\hline
& $=$ & $\subseteq$ & $\leq$ \\
\hline
\textsc{Bgp} & \purple{\bh} / \purple{\thetatwo}  & \sigmatwo / \sigmatwo & \thetatwo / \thetatwo \\
$\pi$-\textsc{Bgp} & \purple{\bh} / \purple{\thetatwo}  & \sigmatwo / \sigmatwo & \thetatwo / \thetatwo \\
\textsc{Wdpt} &\purple{\bh} / \sigmatwo  & \sigmatwo / \sigmatwo & \thetatwo / \sigmatwo \\
$\pi$-\textsc{Wdpt} & \purple{\bh} / \sigmatwo  & \sigmatwo / \sigmatwo & \thetatwo / \sigmatwo \\
\hline
\end{tabular}
\end{table}


We note that in our hardness proofs in Section~\ref{sect:cqa}, we can always choose the target problem instance consisting of a graph $G$, a shape document $(C,T)$, and a set of hypotheses $H$
in such a way that a repair exists. In this case, the \cqa and \mcqa problems coincide. Hence, 
the hardness results of each variant of the \cqa problems carry over to the corresponding variant of the \mcqa. Hence, whenever we manage to show that the membership result for a variant of 
\cqa also holds for the corresponding variant of \mcqa, we may immediately conclude the completeness for this variant of \mcqa.

The algorithms sketched in  Section~\ref{sect:cqa} to prove our membership results for all 
variants of the \cqa problem now have to be extended by ensuring maximum cardinality of the
targets covered by the repair that is guessed as a ``witness'' that the mapping $\mu$ is not, respectively, is a solution of query $q$.
In case of data complexity, we thus have to combine constantly many $\np$-problems 
deciding the question if there exists a repair that covers a subset $T' \subseteq T$ of
cardinality $m$. This requires the power of some level in the Boolean Hierarchy \bh. 
In case of combined complexity, the maximally attainable cardinality of subsets $T' \subseteq T$ allowing for a repair has to be determined by binary search involving logarithmically many 
$\np$-questions of the form ``does there exists a $T' \subseteq T$ with $|T'| \geq m$ such that 
$T'$ allows for a repair?''.  This binary search requires $\Theta_2$-power. 
Hence, for all variants of 
$\cqa$ whose data complexity is at least hard  for every level of $\bh$, 
the membership and, therefore, also the completeness carries over to $\mcqa$. Likewise, 
for all variants of 
$\cqa$ whose combined complexity is at least \thetatwo-hard, the membership and, therefore, also the completeness carries over to $\mcqa$. Hence, in the sequel, we only need to revisit those
cases, where the data complexity is below \bh or the complexity is below \thetatwo.



\subsection{Cautious Reasoning with Max-Repairs}

First, we recall the Boolean hierarchy \bh, which is less common than the other complexity 
classes encountered so far: on the bottom levels, we have \bhone = \np and  \bhtwo = the class of languages obtained as the intersection of a language in \bhone and a language in \conp. 
In other words, we have \bhtwo = \DP. 
For the general case, we have
\bhtwok = the class of languages that are the intersection of a \bhtwokminus language with a 
\conp language and 
\bhtwokplus is the class of languages that are the union of a \bhtwok language with an 
\np language.
% Since \bhk $\subseteq$ \bhkplus holds for every $k$, 
In order to establish membership of a problem in \bh, it suffices to show that 
the problem can be solved in deterministic polynomial time with constantly many 
calls to an \np-oracle. Likewise, to show that a problem is hard for every level of \bh,
it suffices to exhibit a reduction from the 
combinations of $k$ instances of an \np-hard problem 
for arbitrary $k > 0$ asking if all of them have a ``yes'' answer, e.g., 
taking $k$ graphs and asking if all of them are 3-colorable.


\begin{theorem}
\label{thm:max:cautious:equ:data}
\mbgpEqu, \mbgpProjEqu, \mwdptEqu, and \mwdptProjEqu are in \bh data complexity. 
\end{theorem}


\begin{proof}
Consider an arbitrary instance $(G, (C,T), H, q,\mu)$ of 
one of the problems
\mbgpEqu, \mbgpProjEqu, \mwdptEqu, or \mwdptProjEqu. 
Let $|T| = m$.
The question if $\mu$ is {\em not} a solution in every max-repair of 
$G$ w.r.t.\ $((C,T), H)$ can be decided by the following algorithm:

\begin{enumerate}
    \item For every subset $T' \subseteq T$, decide if there exists a repair of 
    $G$ w.r.t., $((C,T'), H)$. 
    \item determine the maximum cardinality $K$ of the subsets $T'$ of $T$ with a ``yes'' answer
    to the above question. 
    \item Check that there exists $T' \subseteq T$ with 
    $|T'| = K$, such that $\mu$ is {\em not} an answer to query $q$ over some repair
    of $G$ w.r.t.\ $((C,T'), H)$.    
\end{enumerate}

For data complexity, $T$ is considered fixed. Hence, there are only constantly many 
subsets $T'$ of $T$ that have to be considered in the first step and each of the questions to be 
answered in the first step are in \np. The second step is then feasible in polynomial time. In order to show that the entire algorithm works in polynomial time with access to constantly many calls to an \np oracle, it suffices to show that the problem to be solved in the third step 
is in \np. Indeed, this problem is a slight variation of the problems
\bgpEqu, \bgpProjEqu, \wdptEqu, and \wdptProjEqu, respectively, in that we now have to 
extend the guess-step by guessing a subset $T'$ of $T$ with $|T'| = K$ and then consider 
repairs w.r.t.\ $((C,T'), H)$ rather than $((C,T), H)$. Clearly, this additional guess does
not destroy the \np-membership of \bgpEqu, \bgpProjEqu, \wdptEqu, and \wdptProjEqu data complexity.
\end{proof}



\begin{theorem}
\label{thm:max:cautious:equ:combined}
\mbgpEqu and  \mwdptEqu are in \thetatwo combined complexity.
\end{theorem}

\begin{proof}
We only need to slightly modify the decision procedure and its complexity analysis from the proof of 
Theorem~\ref{thm:max:cautious:equ:data}. 
First, in combined complexity, the set $T$ is no longer considered as fixed. 
Hence, we now 
determine the maximum cardinality $K$ of subsets $T'$ of $T$ such that 
there exists a repair of $G$ w.r.t., $((C,T'), H)$ by a binary search. That is, 
by asking logarithmically many \np-questions of the form 
``does there exists a subset $T' \subseteq T$ with $|T'| \geq m$ such that  
there exists a repair of $G$ w.r.t. $((C,T'), H)$?''
After that, we need one more oracle call to decide if 
there exists $T' \subseteq T$ with 
$|T'| = K$, such that $\mu$ is {\em not} an answer to query $q$ over some repair
of $G$ w.r.t.\ $((C,T'), H)$. This  oracle call looks the same as the third step in the proof of 
Theorem~\ref{thm:max:cautious:equ:data}. However, for the complexity analysis, 
we have to keep in mind that the query $q$ is no longer considered as fixed. 
This last oracle call is still in \np for BGPs and WDPTs as was shown in 
Section \ref{sect:cqa}. In contrast, 
for $\pi$-BGPs and $\pi$-WDPTs it is not.   
\end{proof}


\subsection{Very Cautious and Brave Reasoning with Max-Repairs}

\begin{theorem}
\label{thm:max:verycautious:equ}
\mbgpEquIn, \mbgpProjEquIn, and \mwdptEquIn are in \bh data complexity. 
Moreover, \mbgpEquIn is in \thetatwo combined complexity. 
\end{theorem}

\begin{proof}
For the data complexity, the \bh-membership is shown analogously to the case of 
cautious reasoning addressed in Theorem~\ref{thm:max:cautious:equ:data}: 
first the maximum cardinality $K$ of the subsets $T'$ of $T$, such that $G$ has a repair
w.r.t.\ \ $((C,T'), H)$ is determined by constantly many calls to an \np-oracle. 
Then it is checked if $\mu$ is an answer to  $q$ in the intersection of all repairs of 
$G$ w.r.t.\ to all combinations of shapes $(C,T')$ and $H$
with $|T| = K$. Analogously to the third step in the proof of 
Theorem~\ref{thm:max:cautious:equ:data}, this check has the 
same complexity as checking
if $\mu$ is an answer to  $q$ in the intersection of all repairs of 
$G$ w.r.t.\ $(C,T)$ and $H$. That is, this check requires 
one more \np-oracle call (due to the \conp-membership of 
\bgpEquIn and \bgpProjEquIn) or two more 
\np-oracle calls (due to the \DP-membership of 
\wdptEquIn), respectively.

For the combined complexity, 
\thetatwo-membership of \mbgpEquIn is shown analogously to 
Theorem~\ref{thm:max:cautious:equ:combined}. That is, we first 
determine the 
the maximum cardinality $K$ of the subsets $T'$ of $T$, such that $G$ has a repair
w.r.t.\ \ $((C,T'), H)$ by means of logarithmically many calls to an 
\np-oracle. And then we need a final \np-oracle call to answer the
question if $\mu$ is {\em not} an answer to $q$ in at least 
one repair of $G$ w.r.t.\ at least one $(C,T'), H)$ with $T' \subseteq T$
and $|T'| = K$.
\end{proof}

\begin{theorem}
\label{thm:max:brave:equ}
\mbgpEquEx, \mbgpProjEquEx,  \mwdptEquEx, and  \mwdptProjEquEx
are in \bh data complexity. 
Moreover, \mbgpEquEx and \mbgpProjEquEx are in \thetatwo combined complexity. 
\end{theorem}

\begin{proof}
For the data complexity, the \bh-membership is shown analogously to the case of 
very cautious reasoning addressed in Theorem~\ref{thm:max:verycautious:equ}: 
first the maximum cardinality $K$ of the subsets $T'$ of $T$, such that $G$ has a repair
w.r.t.\ \ $((C,T'), H)$ is determined by constantly many calls to an \np-oracle. 
Then it is checked if there exists a subset $T' \subseteq T$ with
$|T'| = K$, such that 
$\mu$ is an answer to  $q$ in at least one  repair of 
$G$ w.r.t.\ $((C,T'), H)$. The complexity of this last step is the same as 
the complexity of deciding if $\mu$ is an answer to $q$ in at least
one repair of $G$ w.r.t.\ $((C,T), H)$. Hence, it is in \np in all 4 cases.

Also for the combined complexity, the membership
(in this case, \thetatwo-membership)  of \mbgpEquIn is shown analogously to 
Theorem~\ref{thm:max:cautious:equ:combined}. That is, after determining 
the maximum cardinality $K$ of the subsets $T'$ of $T$, such that $G$ has a repair
w.r.t.\ \ $((C,T'), H)$ by means of logarithmically many \np-oracle calls,
we need a final \np-oracle call to answer the
question if $\mu$ is an answer to $q$ in at least 
one repair of $G$ w.r.t.\ at least one $((C,T'), H)$ with $T' \subseteq T$
and $|T'| = K$.
\end{proof}



